Structure-Adaptive Estimation of Heterogeneous Treatment Effects with Kernel Methods

We study conditional average treatment effect (CATE) estimation from observational data in regimes with potentially weak overlap, when the nuisance response functions lie in a reproducing kernel Hilbert space (RKHS), but the contrast function is structurally simpler. We consider three forms of such simplicity: (i) membership in a lower-complexity RKHS with faster eigenvalue decay, (ii) a source condition relative to the nuisance kernel, or (iii) dependence on a known low-dimensional covariate representation. We develop a unified two-stage kernel ridge regression procedure that remains valid under weak overlap and attains minimax rates determined by the complexity of the contrast function. The procedure avoids propensity-score estimation and separate nuisance convergence-rate assumptions. We also show that a simple model-selection step over candidate contrast spaces and regularization levels satisfies an oracle inequality, enabling adaptation to unknown CATE regularity.

==> macros.tex <==
\makeatletter
\newif\ifucateneurips
\@ifpackageloaded{neurips_2026}{\ucateneuripstrue}{\ucateneuripsfalse}
\newcommand{\UCATEMaybeUsePackage}[2][]{%
  \@ifpackageloaded{#2}{}{\usepackage[#1]{#2}}%
}
\newcommand{\UCATEMaybeRequirePackage}[2][]{%
  \@ifpackageloaded{#2}{}{\RequirePackage[#1]{#2}}%
}
\makeatother

\UCATEMaybeUsePackage[T1]{fontenc}
% \usepackage[latin9]{inputenc}
\ifucateneurips\else
\usepackage{geometry}
\geometry{verbose,tmargin=1in,bmargin=1in,lmargin=1in,rmargin=1in}
\fi
%\usepackage{babel}
\UCATEMaybeUsePackage{verbatim}
\UCATEMaybeUsePackage{float}
\UCATEMaybeUsePackage{bm}
\UCATEMaybeUsePackage{amsmath}
\UCATEMaybeUsePackage{amssymb}
\UCATEMaybeUsePackage{amsfonts}
\UCATEMaybeUsePackage{graphicx}
\ifucateneurips\else
\UCATEMaybeUsePackage{breakurl}
\fi
\UCATEMaybeUsePackage{multirow}
\UCATEMaybeUsePackage{mathtools}
\UCATEMaybeUsePackage{makecell}
\UCATEMaybeUsePackage{xr}
\UCATEMaybeUsePackage{pgfplots}


\UCATEMaybeUsePackage{microtype}
\UCATEMaybeUsePackage{graphicx}
\UCATEMaybeUsePackage{subfigure}
\UCATEMaybeUsePackage{booktabs} % for professional tables
\newcommand{\op}{\operatorname{op}}

%\RequirePackage[numbers]{natbib}
\ifucateneurips\else
\UCATEMaybeRequirePackage[authoryear]{natbib} %% uncomment this for author-year bibliography
\fi
%\RequirePackage{hyperref}
\makeatletter
\@ifpackageloaded{hyperref}{}{%
\PassOptionsToPackage{hyphens}{url}\usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}}
\makeatother

\UCATEMaybeUsePackage{cleveref}
\UCATEMaybeUsePackage{lipsum}
%\usepackage{subcaption}

\makeatletter
\def\blfootnote{\gdef\@thefnmark{}\@footnotetext}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LyX specific LaTeX commands.
%% Because html converters don't know tabularnewline
\providecommand{\tabularnewline}{\\}
\floatstyle{ruled}
%\renewcommand{\baselinestretch} {1.0}
\makeatletter
\@ifundefined{algorithm}{\newfloat{algorithm}{tbp}{loa}}{}
\makeatother
\providecommand{\algorithmname}{Algorithm}
\floatname{algorithm}{\protect\algorithmname}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% User specified LaTeX commands.

\UCATEMaybeUsePackage{amsthm}\UCATEMaybeUsePackage{dsfont}\UCATEMaybeUsePackage{array}\UCATEMaybeUsePackage{mathrsfs}\UCATEMaybeUsePackage{comment}
\ifucateneurips\else
\onecolumn
\fi

\UCATEMaybeUsePackage{color}%\usepackage{babel}
\newcommand{\mypara}[1]{\paragraph{#1.}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\rd}{\mathrm{d}}

\UCATEMaybeUsePackage{enumitem}
\setlist[itemize]{leftmargin=1em}
\setlist[enumerate]{leftmargin=1em}
\allowdisplaybreaks

%\usepackage{babel}
\ifucateneurips\else
\UCATEMaybeUsePackage[algo2e]{algorithm2e}
\fi
\UCATEMaybeUsePackage{algorithmic}
\UCATEMaybeUsePackage{arydshln}
\UCATEMaybeUsePackage{enumitem}


\DeclareRobustCommand{\vec}[1]{\bm{#1}}
\pdfstringdefDisableCommands{%
	\renewcommand{\vec}[1]{#1}%
}



\newcommand{\ab}{\mathbf{a}}
\newcommand{\bbb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\ba}{\bm{a}}
\newcommand{\bb}{\bm{b}}
\newcommand{\bc}{\bm{c}}
\newcommand{\bd}{\bm{d}}
\newcommand{\be}{\bm{e}}
\newcommand{\bbf}{\bm{f}}
\newcommand{\bg}{\bm{g}}
\newcommand{\bh}{\bm{h}}
\newcommand{\bi}{\bmf{i}}
\newcommand{\bj}{\bm{j}}
\newcommand{\bk}{\bm{k}}
\newcommand{\bl}{\bm{l}}
\newcommand{\bbm}{\bm{m}}
\newcommand{\bn}{\bm{n}}
\newcommand{\bo}{\bm{o}}
\newcommand{\bp}{\bm{p}}
\newcommand{\bq}{\bm{q}}
\newcommand{\br}{\bm{r}}
\newcommand{\bs}{\bm{s}}
\newcommand{\bt}{\bm{t}}
\newcommand{\bu}{\bm{u}}
\newcommand{\bv}{\bm{v}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bx}{\bm{x}}
\newcommand{\by}{\bm{y}}
\newcommand{\bz}{\bm{z}}




\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Sb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\bA}{\bm{A}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bC}{\bm{C}}
\newcommand{\bD}{\bm{D}}
\newcommand{\bE}{\bm{E}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bG}{\bm{G}}
\newcommand{\bH}{\bm{H}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bJ}{\bm{J}}
\newcommand{\bK}{\bm{K}}
\newcommand{\bL}{\bm{L}}
\newcommand{\bM}{\bm{M}}
\newcommand{\bN}{\bm{N}}
\newcommand{\bO}{\bm{O}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bQ}{\bm{Q}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bT}{\bm{T}}
\newcommand{\bU}{\bm{U}}
\newcommand{\bV}{\bm{V}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bX}{\bm{X}}
\newcommand{\bY}{\bm{Y}}
\newcommand{\bZ}{\bm{Z}}


%----- calligraphic fonts -----%

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}




%----- blackboard bold fonts-----%

\newcommand{\HH}{\mathbb{H}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\OOmega}{\mathbb{\Omega}}


\newcommand{\Acr}{\mathscr{A}}
\newcommand{\Bcr}{\mathscr{B}}
\newcommand{\Ccr}{\mathscr{C}}
\newcommand{\Dcr}{\mathscr{D}}
\newcommand{\Ecr}{\mathscr{E}}
\newcommand{\Fcr}{\mathscr{F}}
\newcommand{\Gcr}{\mathscr{G}}
\newcommand{\Hcr}{\mathscr{H}}
\newcommand{\Icr}{\mathscr{I}}
\newcommand{\Jcr}{\mathscr{J}}
\newcommand{\Kcr}{\mathscr{K}}
\newcommand{\Lcr}{\mathscr{L}}
\newcommand{\Mcr}{\mathscr{M}}
\newcommand{\Ncr}{\mathscr{N}}
\newcommand{\Ocr}{\mathscr{O}}
\newcommand{\Pcr}{\mathscr{P}}
\newcommand{\Qcr}{\mathscr{Q}}
\newcommand{\Rcr}{\mathscr{R}}
\newcommand{\Scr}{\mathscr{S}}
\newcommand{\Tcr}{\mathscr{T}}
\newcommand{\Ucr}{\mathscr{U}}
\newcommand{\Vcr}{\mathscr{V}}
\newcommand{\Wcr}{\mathscr{W}}
\newcommand{\Xcr}{\mathscr{X}}
\newcommand{\Ycr}{\mathscr{Y}}
\newcommand{\Zcr}{\mathscr{Z}}
\newcommand{\indicator}{\bm{1}}
% bold alphabet 

%----- bold greek fonts -----%

\newcommand{\balpha}{\bm{\alpha}}
\newcommand{\bbeta}{\bm{\beta}}
\newcommand{\bgamma}{\bm{\gamma}}
\newcommand{\bdelta}{\bm{\delta}}
\newcommand{\bepsilon}{\bm{\epsilon}}
\newcommand{\bvarepsilon}{\bm{\varepsilon}}
\newcommand{\bzeta}{\bm{\zeta}}
\newcommand{\btheta}{\bm{\theta}}
\newcommand{\bvartheta}{\bm{\vartheta}}
\newcommand{\bkappa}{\bm{\kappa}}
\newcommand{\blambda}{\bm{\lambda}}
\newcommand{\bmu}{\bm{\mu}}
\newcommand{\bnu}{\bm{\nu}}
\newcommand{\bxi}{\bm{\xi}}
\newcommand{\bpi}{\bm{\pi}}
\newcommand{\bvarpi}{\bm{\varpi}}
\newcommand{\brho}{\bm{\varrho}}
\newcommand{\bsigma}{\bm{\sigma}}
\newcommand{\bvarsigma}{\bm{\varsigma}}
\newcommand{\btau}{\bm{\tau}}
\newcommand{\bupsilon}{\bm{\upsilon}}
\newcommand{\bphi}{\bm{\phi}}
\newcommand{\bvarphi}{\bm{\varphi}}
\newcommand{\bchi}{\bm{\chi}}
\newcommand{\bpsi}{\bm{\psi}}
\newcommand{\bomega}{\bm{\omega}}

\newcommand{\bGamma}{\bm{\Gamma}}
\newcommand{\bDelta}{\bm{\Delta}}
\newcommand{\bTheta}{\bm{\Theta}}
\newcommand{\bLambda}{\bm{\Lambda}}
\newcommand{\bXi}{\bm{\Xi}}
\newcommand{\bPi}{\bm{\Pi}}
\newcommand{\bSigma}{\bm{\Sigma}}
\newcommand{\bUpsilon}{\bm{\Upsilon}}
\newcommand{\bPhi}{\bm{\Phi}}
\newcommand{\bPsi}{\bm{\Psi}}
\newcommand{\bOmega}{\bm{\Omega}}


%----- Some standard definitions -----%

\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\minimize}{\mathop{\mathrm{minimize}}}

\newcommand{\sgn}{\mathop{\mathrm{sgn}}}
\newcommand{\Tr}{\mathop{\mathrm{Tr}}}
\newcommand{\supp}{\mathop{\mathrm{supp}}}

\DeclareMathOperator{\var}{{\rm var}}
\DeclareMathOperator{\cor}{\rm corr}
\DeclareMathOperator{\cov}{\rm cov}
\DeclareMathOperator{\ind}{\mathds{1}}  % Indicator
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}

\newcommand*{\zero}{{\bm 0}}
\newcommand*{\one}{{\bm 1}}

\newcommand{\diag}{{\rm diag}}
\newcommand{\Range}{{\rm Range}}

\newcommand{\Ber}{{\rm Ber}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%% Norms

\newcommand{\norm}[1]{||#1||}
\newcommand{\bignorm}[1]{\bigg|\bigg|#1\bigg|\bigg|}
\newcommand{\opnorm}[2]{| \! | \! | #1 | \! | \! |_{{#2}}}

%%%%% Dot product
\newcommand{\dotp}[2]{\langle{#1},{#2}\rangle}

%%%%  brackets
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}


%%%%%%%%%  Other commands
\newcommand{\tp}{t_{\text{pert}}}
\newcommand{\dist}{\mathsf{d}}
\newcommand{\mcomment}[1]{\marginpar{\tiny{#1}}}
\newcommand{\fcomment}[1]{\footnote{\tiny{#1}}}
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\snr}{\mathrm{SNR}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\risk}{\cR}
\newcommand{\empiricalrisk}{\cR_{\mathrm{in}}}
\newcommand{\functionclass}{\cF}
\newcommand{\diam}{\mathrm{diam}}

\newcommand{\mean}{\mu}
\newcommand{\meanhat}{\widehat{\mu}}
\newcommand{\sd}{\sigma}
\newcommand{\sdhat}{\widehat{\sigma}}
\newcommand{\totalsd}{v}
\newcommand{\totalsdhat}{\widehat{v}}
\newcommand{\distP}{\cP}
\newcommand{\distQ}{\cQ}
\newcommand{\dataset}{\cD}
\newcommand{\datasetB}{\cB}
\newcommand{\loss}{\ell}

\newcommand{\alg}{\cA}
\newcommand{\algtr}{\cT}
\newcommand{\algva}{\cV}


\makeatother


\theoremstyle{plain}
\makeatletter
\@ifundefined{lemma}{\newtheorem{lemma}{\textbf{Lemma}}}{}
\@ifundefined{prop}{\newtheorem{prop}{\textbf{Proposition}}}{}
\@ifundefined{theorem}{\newtheorem{theorem}{\textbf{Theorem}}\setcounter{theorem}{0}}{}
\@ifundefined{corollary}{\newtheorem{corollary}{\textbf{Corollary}}}{}
\@ifundefined{assumption}{\newtheorem{assumption}{\textbf{Assumption}}}{}
\@ifundefined{example}{\newtheorem{example}{\textbf{Example}}}{}
\@ifundefined{definition}{\newtheorem{definition}{\textbf{Definition}}}{}
\@ifundefined{fact}{\newtheorem{fact}{\textbf{Fact}}}{}
\@ifundefined{problem}{\newtheorem{problem}{\textbf{Problem}}}{}
\@ifundefined{proposition}{\newtheorem{proposition}{\textbf{Proposition}}}{}

\theoremstyle{definition}
\@ifundefined{remark}{\newtheorem{remark}{\textbf{Remark}}}{}
\@ifundefined{claim}{\newtheorem{claim}{\textbf{Claim}}}{}
\@ifundefined{conjecture}{\newtheorem{conjecture}{\textbf{Conjecture}}}{}
\@ifundefined{model}{\newtheorem{model}{\textbf{Model}}}{}
\@ifundefined{setup}{\newtheorem{setup}{\textbf{Setup}}}{}
\makeatother



% \numberwithin{equation}{section}
% \numberwithin{theorem}{section}
% \numberwithin{lemma}{section}
% \numberwithin{corollary}{section}
% \numberwithin{claim}{section}
% \numberwithin{fact}{section}
% \numberwithin{definition}{section}
% \numberwithin{example}{section}
% \numberwithin{assumption}{section}
% \numberwithin{problem}{section}

